Robust Stackelberg buyers in repeated auctions

We consider the practical and classical setting where the seller is using an exploration stage to learn the value distributions of the bidders before running a revenue-maximizing auction in a exploitation phase. In this two-stage process, we exhibit practical, simple and robust strategies with large utility uplifts for the bidders. We quantify precisely the seller revenue against non-discounted buyers, complementing recent studies that had focused on impatient/heavily discounted buyers. We also prove the robustness of these shading strategies to sample approximation error of the seller, to bidder's approximation error of the competition and to possible change of the mechanisms.

==> figures/ProofsSec3Thresholding.tex <==
%!TEX root = main.tex
\begin{proof}[Proof of Theorem thm:2StepProcessCommitment]
Cannibalize below. Simple computations. Just add that thresholding below monopoly price is not good as it does not move the reserve price. 

Also, here when $r>\psi^{-1}(0)$, the reserve price in the second phase has no impact as all bids go through. 
\end{proof}

\begin{lemma}[Phase transition]\label{app:lemma:phaseTransition}
Assume the setup of Theorem \ref{thm:2StepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases. 

Then there is a critical value $\alpha_c$ for which, if $\alpha<\alpha_c$, it is preferable for the bidder to threshold and if $\alpha>\alpha_c$, it is preferable for the bidder to bid truthfully. 	
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:phaseTransition}]
When $G_1=G_2=G$, we have ${\mathcal G}_\alpha=G$. Hence $U(r)$ does not depend on $\alpha$, when $r>\psi^{-1}(0)$.  Hence the optimal utility for the seller is independent of $\alpha$; let us call it $U^*(G)$.

On the other hand, we have 
$$
U(0)=\alpha\Exp{(X-\psi(X))G(X)}+(1-\alpha)\Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}\;.
$$
Obviously, $\Exp{(X-\psi(X))G(X)}> \Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}$. Hence $U(0)$ is increasing in $\alpha$. In the rest of the proof we denote $U(0)$ by $U(0;\alpha)$ to stress its dependence on $\alpha$. 

The results for $\alpha=0$ correspond to \cite{nedelec2018thresholding}.  So we know that as $\alpha\tendsto 0$ $U(0;\alpha)<U^*(G)$. Indeed, thresholding at the monopoly price $r=\psi^{-1}(0)$ beats bidding truthful in that case. And optimal thresholding beats thresholding at the monopoly price.  On the other hand, $U(0;\alpha=1)>U^*(G)$ since truthful bidding is optimal when there is no exploitation phase. Since $U(0;\alpha)$ is an increasing function of $\alpha$, and is obviously continuous, we see that there exists a unique $\alpha_c$ such that if $\alpha<\alpha_c$, it is preferable for the buyer to shade her bid and above it, it is preferable to bid truthful. 

\nek{probably needs $\psi^{-1}(0)\neq 0$ somewhere}

\end{proof}
%
% We suppose in this subsection that the seller commits to thresholding. We note that when $r\geq \psi^{-1}(0)$,
% We have the following theorem.
% \begin{theorem}\label{thm:2StepProcessCommitment}
% We call ${\mathcal G}_\gamma=G_1+\gamma G_2$.
% If the buyer uses a $(r,0)$-thresholding strategy and commits to it, we have for their utility, if the seller is welfare benevolent~:
% if $r\geq \psi^{-1}(0)$,
% \begin{equation}
% U(r)=\Exp{X{\mathcal G}_\gamma\left(\frac{r(1-F(r))}{1-F(X)}\right)\indicator{X\leq r}}+\Exp{(X-\psi(X)){\mathcal G}_\gamma(X)\indicator{X\geq r}}\;.
% \end{equation}
% if $r<\psi^{-1}(0)$,
% \begin{equation}
% U(r)=\Exp{X G_1\left(\frac{r(1-F(r))}{1-F(X)}\right)\indicator{X\leq r}}+\Exp{(X-\psi(X))\left[G_1(X)\indicator{X\geq r}+\gamma G_2(X)\indicator{X\geq \psi^{-1}(0)}\right]}\;.
% \end{equation}
%
% This utility has a discontinuity at $r=\psi^{-1}(0)$. For $r<\psi^{-1}(0)$, we have $U(0)\geq U(r)$. For $r>\psi^{-1}(0)$, the first order condition are the same as in \nek{cite our work} where the distribution of the competition is now ${\mathcal G}_\gamma=G_1+\gamma G_2$. Call $r^*(\gamma)$ the unique solution to this problem.
%
% Hence, the optimal threshold is $\argmax_{r\in \{0,r^*_\gamma\}} U(r)$. When the optimal threshold is 0, our bid is truthful, of course.
%
% \end{theorem}
% \begin{proof}
% Cannibalize below. Simple computations. Just add that thresholding below monopoly price is not good as it does not move the reserve price.
%
% Also, here when $r>\psi^{-1}(0)$, the reserve price in the second phase has no impact as all bids go through.
% \end{proof}
%
% \begin{lemma}[Phase transition]\label{lemma:phaseTransition}
% Assume the setup of Theorem \ref{thm:2StepProcessCommitment}. Suppose that $G_1=G_2$, i.e. the distribution of the competition is the same in the two phases.
%
% Then there is a critical value $\gamma_c$ for which, if $\gamma>\gamma_c$, it is preferable for the bidder to threshold and if $\gamma<\gamma_c$, it is preferable for the bidder to bid truthfully.
% \end{lemma}
%
% \begin{proof}
% When $G_1=G_2=G$, we have ${\mathcal G}_\gamma/(1+\gamma)=G$. Hence $U(r)/(1+\gamma)$ does not depend on $\gamma$, when $r>\psi^{-1}(0)$.  Hence the optimal utility for the seller is independent of $\gamma$; let us call it $U^*(G)$.
%
% On the other hand, we have
% $$
% \frac{U(0;\gamma)}{1+\gamma}=\frac{1}{1+\gamma}\Exp{(X-\psi(X))G(X)}+\frac{\gamma}{1+\gamma}\Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}\;.
% $$
% Obviously, $\Exp{(X-\psi(X))G(X)}> \Exp{(X-\psi(X))G(X)\indicator{X\geq \psi^{-1}(0)}}$. Hence $U(0;\gamma)/(1+\gamma)$ is decreasing in $\gamma$.
%
% The results for $\gamma=\infty$ correspond to \nek{cite our papers.}  So we know that as $\gamma\tendsto \infty$ $U(0;\gamma)/(1+\gamma)<U^*(G)$. On the other hand, $U(0;\gamma=0)/1>U^*(G)$ since truthful bidding is optimal when there is no exploitation phase. Since $U(0;\gamma)/(1+\gamma)$ is a decreasing function, and is obviously continuous, we see that there exists a unique $\gamma_c$ such that if $\gamma>\gamma_c$, it is preferable for the buyer to shade her bid and below it, it is preferable to bid truthful.
%
% \end{proof}

% \subsection{Existence of a Nash equilibrium in the two-stage game}
% Our approach here is the following. All players have essentially two strategies, according to Theorem \ref{thm}. They can either threshold optimally above the monopoly price or bid truthfully. We consider the first order conditions for a Nash equilibrium if all players threshold and we then study the best response of the remaining player.
%
% \begin{theorem}
% We consider the symmetric case and assume that the value distribution of the buyer is regular and follows the assumption of Theorem \ref{thm:nashEquiThresholded}.
% There exists $\alpha_{c,\text{thresh}}$ (possibly 0 or $\infty$) such that if $\alpha\leq \alpha_{c,\text{tresh}}$ there exists a symmetric Nash equilibrium in the class of thresholded strategies. It is the same as in the case $\alpha=0$ and the revenue of the bidders is the same as in a second price auction with no reserve.
%
% There exists $\alpha_{c,\text{truthful}}$ (possibly 0 or $\infty$) such that if $\alpha\geq \alpha_{c,\text{truthful}}$ there exists a symmetric Nash equilibrium in the class of thresholded strategies and it corresponds to bidding truthfully.
% \end{theorem}
% We provide more precise characterizations of the critical $\alpha$'s in the Appendix \nek{say where}
\begin{proof}[Proof of Theorem \ref{thm:ExistenceNashEqui2Stage}]
It is clear that each buyer's best response is either to bid truthful or to threshold optimally in the class of strategies we consider. 	

The theorem follows from Lemma \ref{lemma:phaseTransition}.	\textbf{1) Part 1.} For the first part, we suppose that all players except 1 plays the optimal thresholded strategy characterized by $r^*$ the unique solution of the equation 
$$
\frac{K-1}{r(1-F(r))}\Exp{XF^{K-2}(X)(1-F(X))\indicator{X\leq r}}=F^{K-1}(r)\;.
$$
This gives rise to the competition distribution 
$$
G_\beta(x;r^*)=F^{K-1}(\beta^{-1}(x))=\left(1-\frac{r^*(1-F(r^*))}{x}\right)^{K-1}\indicator{r^*(1-F(r^*))\leq x \leq r^*}+F^{K-1}(x)\indicator{x\geq r^*}\;.
$$
According to Lemma \ref{lemma:phaseTransition}, for this distribution $G_\beta(x;r^*)$, there exists $\alpha_{c,\text{thresh}}$ such that if $\alpha<\alpha_{c,\text{thresh}}$, the best response of the buyer in the class we consider is to threshold at $r>\psi^{-1}(0)$. Our results on Nash equilibria \nek{put a reference} in the case $\alpha=0$ \nek{check case no exploration}. By construction the optimal $r$ for this buyer is $r^*$ and we have the Nash equilibrium. 

Of course, if $\alpha>\alpha_{c,\text{thresh}}$, the best response of the buyer is to bid truthfully and hence there cannot be a Nash equilibrium in thresholding above $\psi^{-1}(0)$. 

\textbf{2) Part 2.} If all the players except one bid truthfully, Lemma \ref{lemma:phaseTransition} applies with $G=F^{K-1}$ and says that there exists $\alpha_{c,\text{truthful}}$, such that if $\alpha>\alpha_{c,\text{truthful}}$ the best response of the last player is to bid truthful. Hence there is a Nash equilibrium in the class we consider. On the other hand, if $\alpha<\alpha_{c,\text{truthful}}$, the best response of the last player is to threshold above $\psi^{-1}(0)$ and hence there is no Nash equilibrium. 

	
\end{proof}

